Finding Influential Institutions in Bibliographic Information Networks

Ranking in bibliographic information networks is a widely studied problem due to its many applications such as advertisement industry, funding, search engines, etc. Most of the existing works on ranking in bibliographic information network are based on ranking of research papers and their authors. But the bibliographic information network can be used for solving other important problems as well. The KDD Cup $2016$ competition considers one such problem, which is to measure the impact of research institutions, i.e. to perform ranking of research institutions. The competition took place in three phases. In this paper, we discuss our solutions for ranking institutions in each phase. We participated under team name "anu@TASL" and our solutions achieved the average NDCG@$20$ score of $0.7483$, ranking in eleventh place in the contest.

==> listofitems.tex <==
% Ce fichier contient le code de l'extension "listofitems"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\loiname                 {listofitems}                           %
\def\loiver                      {1.3}                              %
%                                                                    %
\def\loidate                  {2016/11/18}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% --------------------------------------------------------------------
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%
% %     http://www.latex-project.org/lppl.txt
%
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% --------------------------------------------------------------------
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Christian Tellechea
% email: unbonpetit@openmailbox.org
%        Commentaires, suggestions et signalement de bugs bienvenus !
%        Comments, bug reports and suggestions are welcome.
% --------------------------------------------------------------------
% L'extension listofitems est compos\'ee des 7 fichiers suivants :
%   - code               : listofitems            (.tex et .sty)
%   - manuel en francais : listofitems-fr         (.tex et .pdf)
%   - manuel en anglais  : listofitems-en         (.tex et .pdf)
%   - fichier lisezmoi   : README
% --------------------------------------------------------------------
\expandafter\edef\csname loi_restorecatcode\endcsname{\catcode\number`\_=\number\catcode`\_\relax}
\catcode`\_11

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% gestion des erreurs %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\PackageError
	\def\loi_error#1{\PackageError\loiname{#1}{Read the manual}}% pour LaTeX
\else
	\def\loi_error#1{\errmessage{Package \loiname\space Error: #1^^J}}% pour TeX
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% v\'erification de la pr`'esence de etex %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begingroup
\edef\__tempa{\meaning\eTeXversion}\edef\__tempb{\string\eTeXversion}%
\ifx\__tempa\__tempb
	\endgroup
\else
	\endgroup
	\loi_error{You are not using an eTeX engine, listofitems cannot work.}%
	\expandafter\loi_restorecatcode\expandafter\endinput
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macros auxiliaires %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%---- macros de d\'eveloppement et de manipulation d'arguments
\chardef\loi_stop=0
\def\loi_quark{\loi_quark}
\long\def\loi_identity#1{#1}
\def\loi_gobarg#1{}
\long\def\loi_first#1#2{#1}
\long\def\loi_second#1#2{#2}
\long\def\loi_firsttonil#1#2\_nil{#1}
\long\def\loi_antefi#1#2\fi{#2\fi#1}
\long\def\loi_swaparg#1#2{#2{#1}}
\long\def\loi_exparg#1#2{\expandafter\loi_swaparg\expandafter{#2}{#1}}
\long\def\loi_expafternil#1\_nil{\begingroup\def\loi_temp{\endgroup#1}\expandafter\loi_temp}
\def\loi_macroname{\loi_ifinrange\escapechar[[0:255]]{\expandafter\loi_gobarg}{}\string}
\def\loi_argcsname#1#{\begingroup\def\loi_temp{\endgroup#1}\loi_argcsname_i}
\def\loi_argcsname_i#1{\expandafter\loi_temp\csname#1\endcsname}

%--- macros de test
\def\loi_ifnum#1{\ifnum#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifx#1{\ifx#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifempty#1{\loi_exparg\loi_ifx{\expandafter\relax\detokenize{#1}\relax}}
\def\loi_ifstar#1#2{\def\loi_ifstar_i{\loi_ifx{*\loi_nxttok}{\loi_first{#1}}{#2}}\futurelet\loi_nxttok\loi_ifstar_i}
\long\def\loi_ifcs#1{% #1 est-il une sc ?
	\loi_ifempty{#1}
		\loi_second% si #1 est vide, faux
		{\loi_ifspacefirst{#1}
			\loi_second% si espace en 1er, faux
			{\loi_exparg\loi_ifempty{\loi_gobarg#1}% 1 seul token ?
				{\begingroup \escapechar`\_
					\if\expandafter\loi_firsttonil\string#1\_nil\expandafter\loi_firsttonil\string\relax\_nil
						\endgroup\expandafter\loi_first
					\else
						\endgroup\expandafter\loi_second
					\fi
				}
				\loi_second% si plusieurs tokens, faux
			}%
		}%
}
\def\loi_ifinrange#1[[#2:#3]]{\loi_ifnum{\numexpr(#1-#2)*(#1-#3)>0 }\loi_second\loi_first}

%--- macro de type for
%      Voir codes 150 \`a 155 ici --> http://progtex.fr/wp-content/uploads/2014/09/code.txt
%      et pages 175 \`a 184 du livre "Apprendre \`a programmer en TeX"
\def\loi_fornum#1=#2to#3\do{%
	\edef#1{\number\numexpr#2}\edef\loi_sgncmp{\ifnum#1<\numexpr#3\relax>+\else<-\fi}%
	\loi_argcsname\loi_fornum_i{loi_fornum_\string#1\expandafter}\expandafter{\number\numexpr#3\expandafter}\loi_sgncmp#1%
}
\long\def\loi_fornum_i#1#2#3#4#5#6{\def#1{\unless\ifnum#5#3#2\relax\loi_antefi{#6\edef#5{\number\numexpr#5#41\relax}#1}\fi}#1}

%--- macros retirant les espaces extr\^emes
%      Voir codes 320 \`a 324 ici --> http://progtex.fr/wp-content/uploads/2014/09/code.txt
%      et pages 339 \`a 343 de "Apprendre \`a programmer en TeX"
\long\def\loi_ifspacefirst#1{\expandafter\loi_ifspacefirst_i\detokenize{#10} \_nil}
\long\def\loi_ifspacefirst_i#1 #2\_nil{\loi_ifempty{#1}}
\expandafter\def\expandafter\loi_gobspace\space{}
\def\loi_removefirstspaces{\romannumeral\loi_removefirstspaces_i}
\long\def\loi_removefirstspaces_i#1{\loi_ifspacefirst{#1}{\expandafter\loi_removefirstspaces_i\expandafter{\loi_gobspace#1}}{\loi_stop#1}}
\edef\loi_restorezerocatcode{\catcode0=\number\catcode0 \relax}
\catcode0 12
\long\def\loi_removelastspaces#1{\romannumeral\loi_removelastspaces_i#1^^00 ^^00\_nil}
\long\def\loi_removelastspaces_i#1 ^^00{\loi_removelastspaces_ii#1^^00}
\long\def\loi_removelastspaces_ii#1^^00#2\_nil{\loi_ifspacefirst{#2}{\loi_removelastspaces_i#1^^00 ^^00\_nil}{\loi_stop#1}}
\loi_restorezerocatcode
\long\def\loi_removeextremespaces#1{% #1=texte o\`u les espaces extr\^emes sont retir\'es
	\romannumeral\expandafter\expandafter\expandafter\loi_removelastspaces\expandafter\expandafter\expandafter
	{\expandafter\expandafter\expandafter\loi_stop\loi_removefirstspaces{#1}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro publique \setsepchar %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\setsepchar{\futurelet\loi_nxttok\setsepchar_i}
\def\setsepchar_i{\loi_ifx{[\loi_nxttok}\setsepchar_ii{\setsepchar_ii[/]}}
\long\def\setsepchar_ii[#1]#2{% #1=sepcar de <liste des sepcar>  #2=<liste des sepcar>
	\loi_ifempty{#1}
		{\loi_error{Empty separator not allowed, separator "/" used}%
		\setsepchar_ii[/]{#2}%
		}
		{\def\loi_currentsep{#1}%
		\_removeextremespacesfalse
		\loi_nestcnt1 % r\'einitaliser niveau initial \`a 1
		\def\nestdepth{1}%
		\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
		\def\loi_listname{loi_listofsep}%
		\let\loi_def\def \let\loi_edef\edef \let\loi_let\let
		\loi_ifempty{#2}
			{\loi_error{Empty list of separators not allowed, "," used}%
			\readlist_iv1{,}%
			}
			{\readlist_iv1{#2}}%
		\loi_argcsname\let\nestdepth{loi_listofseplen[0]}%
		\loi_argcsname\let\loi_currentsep{loi_listofsep[1]}% 1er car de s\'eparation
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro normalisant l'index %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_normalizeindex#1#2#3{% #1=macroname  #2=liste d'index  #3=profondeur max --> renvoie {err}{indx norm}
	\loi_ifempty{#2}
		{\loi_stop{}{}}
		{\loi_normalizeindex_i1{}{#3}{#1}#2,\loi_quark,}%
}%
\def\loi_normalizeindex_i#1#2#3#4#5,{% #1=compteur de profondeur #2=index pr\'ec\'edents  #3=profondeur max #4=macroname  #5=index courant
	\loi_ifx{\loi_quark#5}
		{\loi_normalizeindex_iii#2\loi_quark}% supprimer la derni\`ere virgule
		{\loi_ifnum{#1>#3 }
			{\loi_invalidindex{Too deeply nested index, index [.] retained}{#2}}% si profondeur trop grande
			{\loi_ifinrange\ifnum\numexpr#5<0 -1*\fi(#5)[[1:\csname #4len[#20]\endcsname]]% si abs(#5) hors de [1,len]
				{\loi_exparg\loi_normalizeindex_ii{\number\numexpr#5\ifnum\numexpr#5<0 +\csname #4len[#20]\endcsname+1\fi}{#1}{#2}{#3}{#4}}
				{\loi_invalidindex{#5 is an invalid index, index [.] retained}{#2}}%
			}%
		}%
}
\def\loi_normalizeindex_ii#1#2#3{\loi_exparg\loi_normalizeindex_i{\number\numexpr#2+1}{#3#1,}}% #1=index \`a rajouter  #2=compteur de profondeur #3=index pr\'ec\'edents
\def\loi_normalizeindex_iii#1,\loi_quark{\loi_stop{}{#1}}
\def\loi_invalidindex#1#2{\loi_ifempty{#2}{\loi_invalidindex_i{#1},}\loi_invalidindex_i{#1}{#2}}
\def\loi_invalidindex_i#1#2{\loi_invalidindex_ii#1\loi_quark#2\loi_quark}
\def\loi_invalidindex_ii#1[.]#2\loi_quark#3,\loi_quark#4\loi_quark,{\loi_stop{#1[#3]#2}{#3}}% #4= index ignor\'es

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% macro publique \readlist %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcount\loi_nestcnt
\def\greadlist{%
	\let\loi_def\gdef \let\loi_edef\xdef \def\loi_let{\global\let}%
	\loi_nestcnt1 % niveau initial = 1
	\loi_argcsname\loi_let{loi_previndex[\number\loi_nestcnt]}\empty
	\loi_ifstar{\_removeextremespacestrue\readlist_i}{\_removeextremespacesfalse\readlist_i}%
}
\def\readlist{%
	\let\loi_def\def \let\loi_edef\edef \let\loi_let\let
	\loi_nestcnt1 % niveau initial = 1
	\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
	\loi_ifstar{\_removeextremespacestrue\readlist_i}{\_removeextremespacesfalse\readlist_i}%
}
\long\def\readlist_i#1#2{% #1=macro stockant les \'el\'ements  #2=liste des \'el\'ements
	\loi_ifcs{#2}
		{\loi_exparg{\readlist_i#1}{#2}}
		{\loi_edef\loi_listname{\loi_macroname#1}%
		\loi_argcsname\loi_let{\loi_listname nest}\nestdepth
		\loi_argcsname\loi_def{\loi_listname[]}{#2}% la liste enti\`ere
		\loi_argcsname\loi_def{\loi_listname sep[]}{}% s\'eparateur vide
		\loi_ifempty{#2}
			{\loi_def#1[##1]{}%
			\loi_argcsname\loi_def{\loi_listname len}{0}\loi_argcsname\loi_def{\loi_listname len[0]}{0}%
			\loi_error{Empty list ignored, nothing to do}%
			}
			{\loi_edef#1[##1]{\unexpanded{\romannumeral\expandafter\loi_auxmacrolistitem\romannumeral\loi_normalizeindex}{\loi_listname}{##1}{\csname\loi_listname nest\endcsname}{\loi_listname}}%
			\loi_argcsname\loi_edef{\loi_listname sep}[##1]{\unexpanded{\romannumeral\expandafter\loi_auxmacrolistitem\romannumeral\loi_normalizeindex}{\loi_listname}{##1}{\csname\loi_listname nest\endcsname}{\loi_listname sep}}%
			\readlist_ii{#2}%
			\loi_argcsname\loi_argcsname\loi_let{\loi_listname len}{\loi_listname len[0]}% longueur du niveau 0
			}%
		}%
}
\def\loi_auxmacrolistitem#1#2#3{%
	\expandafter\expandafter\expandafter\loi_stop\csname#3[#2]\expandafter\endcsname
	\romannumeral\loi_ifempty{#1}{\loi_stop}{\loi_stop\loi_error{#1}}%
}
\def\readlist_ii{%
	\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
	\expandafter\readlist_iii\loi_currentsep||\_nil
}
\long\def\readlist_iii#1||#2\_nil#3{\readlist_iv1{#3#1}}% #1=<sep courant simple>  #3=liste -> rajoute un \'el\'ement vide pour le test ifempty ci dessous
\long\def\readlist_iv#1#2{% #1=compteur d'index  #2=liste d'\'el\'ements \`a examiner
	\loi_ifempty{#2}
		{\loi_argcsname\loi_edef{\loi_listname len[\csname loi_previndex[\number\loi_nestcnt]\endcsname0]}{\number\numexpr#1-1\relax}%
		\advance\loi_nestcnt-1
		\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
		}
		{\loi_expafternil\readlist_vi{#2}{}\_nil\loi_currentsep||\loi_quark||#2\_nil{#1}}% aller isoler le 1er item
}
\long\def\readlist_v#1#2{\readlist_vi{#2}{}#1||\loi_quark||#2\_nil}% #1=liste s\'eparateurs (s\'ep=||)  #2=chaine de tokens
\long\def\readlist_vi#1#2#3||{% #1=liste restante   #2=dernier <sep utile>  #3=<sep courant>
	\loi_ifx{\loi_quark#3}
		{\loi_ifempty{#2}% si #1 vide, aucun <sep utile> n'a \'et\'e trouv\'e, il reste \`a lire "<liste compl\`ete>\_nil"
			{\long\def\readlist_vii##1\_nil##2{\loi_exparg{\readlist_ix{##2}{}}{\loi_gobarg##1}{#2}}}% ##2=compteur d'index
			{\long\def\readlist_vii##1#2{\loi_exparg\readlist_viii{\loi_gobarg##1}\relax}%
			\long\def\readlist_viii##1##2\_nil##3{\loi_exparg{\readlist_ix{##3}}{\loi_gobarg##2}{##1}{#2}}% ##3=compteur d'index
			}%
		\readlist_vii\relax% le \relax meuble l'argument d\'elimit\'e
		}
		{\long\def\readlist_vii##1#3##2\_nil{%
			\loi_ifempty{##2}% si <liste restante> ne contient pas le <sep courant>
				{\readlist_vi{#1}{#2}}% recommencer avec le m\^eme <sep utile>
				{\readlist_vi{##1#3}{#3}}% sinon raccourcir <liste restante> et <sep courant>:=<sep utile>
			}%
		\readlist_vii#1#3\_nil
		}%
}
\long\def\readlist_ix#1#2#3{% #1=compteur d'index  #2=liste restante  #3=\'el\'ement courant
	\loi_ifnum{0\loi_exparg\loi_ifspacefirst{\loi_currentsep}{}1\if_removeextremespaces1\fi=11 }% s'il faur retirer les espaces extr\^emes
		{\loi_exparg{\loi_exparg{\readlist_x{#1}{#2}}}{\loi_removeextremespaces{#3}}}% red\'efinir l'\'el\'ement courant
		{\readlist_x{#1}{#2}{#3}}%
}
\long\def\readlist_x#1#2#3#4{% #1=compteur d'index  #2=liste restante  #3=\'el\'ement courant   #4=sep utilis\'e
	\loi_ifnum{0\if_ignoreemptyitems1\fi\loi_ifempty{#3}1{}=11 }
		{\readlist_iv{#1}{#2}}% si l'on n'ignore pas les \'el\'ements vides :
		{\loi_argcsname\loi_def{\loi_listname[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#3}% assignation de l'item ctuel \`a la macro
		\loi_argcsname\loi_def{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#4}% assignation du <sep> actuel \`a la macro \<macrolist>sep
		\loi_ifnum{\loi_nestcnt<\nestdepth\relax}% si imbrication max non atteinte
			{\advance\loi_nestcnt1
			\loi_argcsname\edef{loi_previndex[\number\loi_nestcnt]}{\csname loi_previndex[\number\numexpr\loi_nestcnt-1]\endcsname#1,}%
			\readlist_ii{#3}% recommencer avec l'\'el\'ement courant
			}
			{}%
		\loi_exparg\readlist_iv{\number\numexpr#1+1}{#2}% puis chercher l'\'el\'ement suivant dans la liste restante
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \listlen %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\listlen#1[#2]{%
	\romannumeral\loi_ifempty{#2}
		{\expandafter\expandafter\expandafter\loi_stop\csname\loi_macroname#1len[0]\endcsname}
		{\loi_exparg\listlen_i{\romannumeral-`\.\loi_macroname#1}{#2}}%
}
\def\listlen_i#1#2{% #1=macro name   #2=index non normalis\'e    prendre <profondeur max-1>
	\loi_exparg{\expandafter\listlen_ii\romannumeral\loi_normalizeindex{#1}{#2}}{\number\numexpr\csname#1nest\endcsname-1}{#1}%
}
\def\listlen_ii#1#2#3{% #1=err   #2=index normalis\'e  #3=macroname
	\expandafter\expandafter\expandafter\loi_stop\csname#3len[#2,0]\expandafter\endcsname
	\romannumeral\loi_ifempty{#1}{\loi_stop}{\loi_stop\loi_error{#1}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \foreachitem %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\foreachitem#1\in#2{%
	\edef\foreachitem_i{\noexpand\foreachitem_iii\noexpand#1{\expandafter\noexpand\csname\loi_macroname#1cnt\endcsname}{\loi_macroname#2}}%
	\futurelet\loi_nxttok\foreachitem_ii
}
\def\foreachitem_ii{\loi_ifx{\loi_nxttok[}\foreachitem_i{\foreachitem_i[]}}
\def\foreachitem_iii#1#2#3[#4]{% prendre <profondeur max-1>
	\loi_exparg{\expandafter\foreachitem_iv\romannumeral\loi_normalizeindex{#3}{#4}}{\number\numexpr\csname#3nest\endcsname-1}#1{#2}{#3}%
}
\def\foreachitem_iv#1#2{\loi_ifempty{#2}{\foreachitem_v{#1}{}}{\foreachitem_v{#1}{#2,}}}% #1=err  #2=index norm
\long\def\foreachitem_v#1#2#3#4#5#6{% #1=err  #2=index norm  #3=macroiter  #4=compteur associ\'e  #5=nom de macrolist  #6=code
	\loi_ifnum{\csname#5len[#20]\endcsname>0 }
		{\loi_ifempty{#1}{}{\loi_error{#1}}%
		\loi_fornum#4=1to\csname#5len[#20]\endcsname\do{\loi_argcsname\let#3{#5[#2#4]}#6}%
		}
		{}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \showitem %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\showitems{\loi_ifstar{\let\showitems_cmd\detokenize\showitems_i}{\let\showitems_cmd\loi_identity\showitems_i}}
\def\showitems_i#1{\def\showitems_ii{\showitems_iv#1}\futurelet\loi_nxttok\showitems_iii}
\def\showitems_iii{\loi_ifx{\loi_nxttok[}\showitems_ii{\showitems_ii[]}}
\def\showitems_iv#1[#2]{\foreachitem\showitems_iter\in#1[#2]{\showitemsmacro{\expandafter\showitems_cmd\expandafter{\showitems_iter}}}}
\unless\ifdefined\fbox
	\newdimen\fboxrule \newdimen\fboxsep \fboxrule=.4pt \fboxsep=3pt % r\'eglages identiques \`a LaTeX
	\def\fbox#1{% imitation de la macro \fbox de LaTeX, voir codes 251 \`a 254 ici --> http://progtex.fr/wp-content/uploads/2014/09/code.txt
		\hbox{% et pages 271 \`a 274 de "Apprendre \`a programmer en TeX"
			\vrule width\fboxrule
			\vtop{%
				\vbox{\hrule height\fboxrule \kern\fboxsep \hbox{\kern\fboxsep#1\kern\fboxsep}}%
				\kern\fboxsep \hrule height\fboxrule
			}\vrule width\fboxrule
		}%
	}
\fi
\def\showitemsmacro#1{% encadrement par d\'efaut
	\begingroup\fboxsep=0.25pt \fboxrule=0.5pt \fbox{\strut#1}\endgroup
	\hskip0.25em\relax
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \itemtomacro %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\itemtomacro#1[#2]{% #1[#2]=item  non encore lu: #3=macro
	\edef\loi_listname{\loi_macroname#1}%
	\loi_exparg{\expandafter\itemtomacro_i\romannumeral\expandafter\loi_normalizeindex\expandafter{\loi_listname}{#2}}{\csname\loi_listname nest\endcsname}\let
}
\def\gitemtomacro#1[#2]{% #1[#2]=item
	\xdef\loi_listname{\loi_macroname#1}%
	\loi_exparg{\expandafter\itemtomacro_i\romannumeral\expandafter\loi_normalizeindex\expandafter{\loi_listname}{#2}}{\csname\loi_listname nest\endcsname}{\global\let}%
}
\def\itemtomacro_i#1#2#3#4{%
	\loi_ifempty{#1}{}{\loi_error{#1}}%
	\loi_argcsname#3#4{\loi_listname[#2]}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%% r\'eglages par d\'efaut %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if_removeextremespaces
\newif\if_ignoreemptyitems
\let\ignoreemptyitems\_ignoreemptyitemstrue
\let\reademptyitems\_ignoreemptyitemsfalse
\setsepchar{,}
\reademptyitems

\loi_restorecatcode
\endinput

######################################################################
#                             Historique                             #
######################################################################

v1.0  19/8/2016
      - Premi\`ere version publique

v1.1  01/09/2016
      - Stockage des s\'eparateurs dans <macrolist>sep
      - bug corrig\'e dans \loi_restorecatcode

v1.2  22/10/2016
      - macros \greadlist et \gitemtomacro pour la globalit\'e

v1.3  18/11/2016
      - bugs corrig\'es dans la gestion de la globalit\'e
